An architecture for non-invasive software measurement

Analysis of data related to software development helps to increase quality, control and predictability of software development processes and products.However, collecting such data for is a complex task. A non-invasive collection of software metrics is one of the most promising approaches to solve the task. In this paper we present an approach which consists of four parts: collect the data, store all collected data, unify the stored data and analyze the data to provide insights to the user about software product or process. We employ the approach to the development of an architecture for non-invasive software measurement system and explain its advantages and limitations.

==> relatedWorks.tex <==
\section{Related works in architectures for non-invasive measurement systems }

Over the past ten years several non-invasive measurement systems have been developed. In this section we review the following systems with emphasis on architecture: 
\begin{itemize}
\item PRO Metrics (PROM);
\item ElectroCodeoGram (ECG);
\item Empirical Project Monitor (EPM); 
\item Hackystat. 
\end{itemize}

\subsection{PRO Metrics }

PRO Metrics \cite{sillitti2003collecting,scotto2006non,sillitti2006managing} is a distributed architecture for collecting software metrics and Personal Software Process (PSP) data. PROM is based on Package-Oriented Programming development technique. Client application stores collected information in XML file and doesn’t deal with transmission task. This decision makes client-side components simpler. A transfer tool is separate client-application that transfers collected data and provides user authentication. 
Server-side components need to be installed and maintain only on one machine, therefore the overall complexity of the system is low. But in case of installation client components on many machines with different environment it becomes not a trivial task for a system administrator.

\subsection{ElectroCodeoGram} 

ElectroCodeoGram is a modular framework \cite{schlesinger2006electrocodeogram} aimed at micro-process research and discovering patterns in the sequence of events which describe the same programming behavior. For instance (i) copy and paste some piece of code with desired functionality and (ii) refactor code and make a function with needed parameters, represent two different patterns (or episodes) solving the same task. ECG is a system which supports micro-process research. It automatically records micro-process data using ECG Sensors; sends data to the central collection and analysis system. Data is transported over network sockets or SOAP. 

\subsection{Empirical Project Monitor}

Empirical Project Monitor \cite{ohira2004empirical,ohira2004empiricalsyst} a system that automatically collects data (by ”pulling”) from three different repositories: 
\begin{itemize}
\item Configuration management systems;
\item Mailing list managers (e.g. Mailman, Majordomo);
\item Issue tracking systems (e.g. Bugzilla).
\end{itemize}


The EPM system consist of three components 
\begin{itemize}
\item Automatic data collection. EMP automatically collects data from repositories mentioned above. 
\item Format translation and data store. EMP converts collected data to XML format. Converted data is stored in the PostgreSQL database. 
\item Analysis and visualization. EPM gets data for analysis from the database. Visualization is a web based application. 
\end{itemize}

\subsection{Hackystat}

Hackystat \cite{johnson2003beyond,johnson2007requirement,johnson2004practical} is a system for automatic collecting development metrics from sensors (attached to development tools).  Hackystat sends data to the server where this data is analyzed. In the first version of Hackystat, its sensors were able to collect: 

\begin{itemize}
\item activity data (e.g. which file is under modification of developer at 30 seconds interval); 
\item size data (e.g. lines of code);
\item defect data (e.g. number of pass/fail status of unit tests).
\end{itemize}

A developer should install one or more sensors to begin using Hackystat and then register with its server. In later versions of Hackystat it architecture has been criticised for growing complexity; developers made a decision to review the architecture and reimplement Hackystat in a service-oriented architecture (SOA). The main challenges for this revision were almost complete reimplementation of the system and the need for system developers to learn new architectural concept and libraries. 

